Fractional Parallel Plate DB Waveguides Using Fractional Curl Operator

DB boundary conditions have been simulated in terms of perfect electric conductor (PEC) boundary for transverse electric modes and perfect magnetic conductor (PMC) for transverse magnetic modes. Electric and magnetic fields inside the dielectric region of a parallel plate DB boundary waveguide have been derived and fractional curl operator has been utilized to study the fractional parallel plate DB waveguide. Field behavior as well as transverse impedance of the guide walls have been studied with respect to the fractional parameter describing the order of fractional curl operator. The results are also compared with the corresponding results for fractional waveguides with PEC walls.

==> PROJFORM.TEX <==
% The File projform.TeX was created on 24th Dec. 1993.
\magnification=1200
\baselineskip=24 truept plus1pt minus1pt
\parskip=9 true pt
\hoffset=0.5 true in
\hsize=6.2 true in
\nopagenumbers
%section headings in bold \section{ }
\def\section#1{\goodbreak\medbreak\noindent{\tenbf #1}\nobreak\smallskip}
%subsection heading in bold \subsection{ }
\def\subsection#1{\goodbreak\smallbreak\noindent{\bf#1}\nobreak\smallskip}
%1 ref# 2 authur 3 title 4 journal name 5vol 6 page,(yr) \ref{1}{2}{3}{4}{5}{6}
\def\ref#1#2#3#4#5#6{\medbreak\noindent\item{#1}{#2},\ {#3}\
{\it #4}{#5}{#6}}
%1 ref# 2 authur 3 name of book 4 publisher,city pub.,(yr) \refbk{1}{2}{3}{4}
\def\refbk#1#2#3#4{\medbreak\noindent\item{#1}{#2},\ {\it #3}\ {#4}}
%Define fonts.
\font\smsl=cmsl8 \font\bigbold=cmbx10 scaled\magstep1
\font\vbigbold=cmbx10 scaled\magstep2
%uppercase roman numeral \romone
\def\romone{\uppercase\expandafter{\romannumeral 1}}
\def\romtwo{\uppercase\expandafter{\romannumeral 2}}
\def\romtre{\uppercase\expandafter{\romannumeral 3}}
\def\romfor{\uppercase\expandafter{\romannumeral 4}}
\def\romfiv{\uppercase\expandafter{\romannumeral 5}}
\def\romsix{\uppercase\expandafter{\romannumeral 6}}
\def\romsev{\uppercase\expandafter{\romannumeral 7}}
\def\romeig{\uppercase\expandafter{\romannumeral 8}}
\def\romnin{\uppercase\expandafter{\romannumeral 9}}
%full page skip for figures \beginfl\vfill
\def\beginfl{\pageinsert\baselineskip 16truept}
%caption for the figure \caption FIGURE ... ! fig. caption... !
\def\caption #1! #2!{\noindent{\bf #1\enspace}{\sl #2}}
%end command for the page skip \endf
\def\endf{\endinsert\baselineskip 24truept}
%line filling with dots,table of contents,no indentation \toclin1{ } {page}
\def\toclin1#1#2{\line{\noindent #1\ \dotfill\ #2}}
%line filling with dots w/indentation \toclin2{ } {page}
\def\toclin2#1#2{\line{\indent #1\ \dotfill\ #2}}
\def\vE{{\bf E}}
\def\vH{{\bf H}}
\def\vB{{\bf B}}
\def\vD{{\bf D}}
\def\vJ{{\bf J}}
\def\vK{{\bf K}}
\def\vN{{\bf N}}
\def\vA{{\bf A}}
\def\vS{{\bf S}}
\def\vV{{\bf V}}
\def\vr{{\bf r}}
\def\va{{\bf a}}
\def\vb{{\bf b}}
\def\ex{{\bf e}_x}
\def\ey{{\bf e}_y}
\def\ez{{\bf e}_z}
%\def\exp{{\bf e}_{x'}}
\def\eyp{{\bf e}_{y'}}
\def\ezp{{\bf e}_{z'}}
\def\er{{\bf e}_r}
\def\erp{{\bf e}_{r'}}
\def\ephi{{\bf e}_\phi}
\def\ephp{{\bf e}_{\phi'}}
\def\et{{\bf e}_\theta}
\def\etp{{\bf e}_{\theta'}}
\endinput
\

